IDNet: Smartphone-based Gait Recognition with Convolutional Neural Networks

Here, we present IDNet, a user authentication framework from smartphone-acquired motion signals. Its goal is to recognize a target user from their way of walking, using the accelerometer and gyroscope (inertial) signals provided by a commercial smartphone worn in the front pocket of the user's trousers. IDNet features several innovations including: i) a robust and smartphone-orientation-independent walking cycle extraction block, ii) a novel feature extractor based on convolutional neural networks, iii) a one-class support vector machine to classify walking cycles, and the coherent integration of these into iv) a multi-stage authentication technique. IDNet is the first system that exploits a deep learning approach as universal feature extractors for gait recognition, and that combines classification results from subsequent walking cycles into a multi-stage decision making framework. Experimental results show the superiority of our approach against state-of-the-art techniques, leading to misclassification rates (either false negatives or positives) smaller than 0.15% with fewer than five walking cycles. Design choices are discussed and motivated throughout, assessing their impact on the user authentication performance.

==> 3_tmp.tex <==
%!TEX root = article.tex

\section{Signal Processing Framework}
\label{sec:signal_acquisition_and_processing}

Next, we present our signal processing framework. Our aim is to correctly recognize a subject from his/her way of walking, through the acquisition of inertial signals from a standard  smartphone. 

%\begin{figure}[!t]
%	\centering
%	\includegraphics[width=8cm]{img/ML_approach.eps}
%	\caption{Classical machine learning approach.}
%	\label{fig:classical_machine_learning}
%\end{figure}

The processing workflow is shown in \fig{fig:processing_workflow}. Walking data is first acquired (see \sect{sec:data_acquisition}), then we perform some preprocessing entailing: 1) pre-filtering to remove motion artefacts (see again \sect{sec:data_acquisition}), 2) a transformation to move the raw walking data into a new {\it orientation independent} reference system, 3) the extraction of walking cycles (\sect{sec:cycle_extraction}), 4) a normalization to represent each walking cycle (accelerometer and gyroscope data) through a fixed length, zero mean and unit variance vector (\sect{sec:normalization}). After this, the walking cycles are ready to be processed to identify the user. The standard approach, called ``Classical Machine Learning'' entails the computation of a number of pre-established statistical features, the most informative of which are selected and used to train a classifier. Various machine learning techniques are usually exploited to this purpose, and are trained through a supervised approach. Hence, the classification performance is assessed and the whole process is usually iterated for a further feature selection phase. In this way, we progressively refine the features that are used for the classification task until a final feature set is attained. Note that statistical features are often assessed by the designer through educated guesses.  

As opposed to this, in this paper we advocate the use of convolutional neural networks (\sect{sec:conv_neural_net}). These have been successfully used by the video processing community~\cite{CNN_video_analysis_2014} but to the best of our knowledge have never been exploited for the analysis of inertial data from wearable devices. One of the main advantages of this approach is that statistical features are automatically assessed by the CNN as a result of a supervised training phase. As we shall see shortly, this automatic feature engineering has a much higher discriminative power, which allows for better classification results. 

The processing blocks are described in higher details in the following subsections.\\

\noindent \textbf{Notation:} With $\pmb{x} \in \mathbb{R}^n$ we mean a column vector $\pmb{x}=(x_1,x_2,\dots,x_n)^T$ with elements $x_i \in \mathbb{R}$. $|\pmb{x}|=n$ returns the number of elements in $\pmb{x}$. $\bar{\pmb{x}}=(\sum_{i=1}^n x_i)/n$, whereas $\|\pmb{x}\|=(\sum_{i=1}^n x_i^2)^{1/2}$ is the L2-norm operator. If $\pmb{x}, \pmb{y} \in \mathbb{R}^n$, we define their inner product as $\pmb{x} \cdot \pmb{y} = \pmb{x}^T \pmb{y}$ and their entrywise product as $\pmb{x} \circ \pmb{y} = (x_1 y_1, x_2 y_2, \dots, x_n y_n)^T$. With $\vec{\pmb{r}}$ we mean a 3D vector $\vec{\pmb{r}}=(r_1,r_2,r_3)^T$ and $\hat{\pmb{r}}$ is the corresponding 3D versor $\hat{\pmb{r}}=\vec{\pmb{r}}/\|\vec{\pmb{r}}\|$. With any two 3D vectors $\vec{\pmb{r}}$ and $\vec{\pmb{s}}$ we indicate their cross-product as $\vec{\pmb{r}} \times \vec{\pmb{s}} = (r_2 s_3 - r_3 s_2, r_3 s_1 - r_1 s_3, r_1 s_2 - r_2 s_1)^T$. With $u(i)$ we mean a time series, where $i=1,2,\dots$ is the discrete time index.  

\subsection{Data Acquisition and Filtering}
\label{sec:data_acquisition}

%When a learning approach is used, the quality of data is one of the most important factor to obtain good results. For this reason we decided to create our dataset, acquiring data directly from users, in a controlled but as real as possible environment.
%Inertial data acquired holding the smartphone in the trouser's pocket is poorly studied for walking analysis. So the following step is the analysis of data, in order to understand the relationship between the gait cycle and the acquired signals, and to optimize a first preprocessing phase.
%As introduced in~\sect{related_work}, two type of windowing method can be used: fixed time or cycles based. Cycles based approach can be considered a dynamic windowing method, in which the length of the window correspond to the current gait cycle duration. We consider fixed time windowing, although very simple, a poor approach to this problem, mainly due to the variability in walking speed, both for intra-class and inter-class data. A real-time cycle extraction algorithm is then required.
%In order to make a system independent to respect to the orientation, we implement a coordinates transformation. It isn't possible to know the smartphone position inside the pocket, then we need to extract the new reference system directly from data.
%ML approach is compared with an intelligent system, that uses convolutional network, for feature extraction phase, that is the process that transforms original input signals into a new space of variables where the pattern recognition problem is easier to solve. To reduce the number of variables for ML algorithm, a feature selection phase is often considered.
%There aren't rules regarding the choice of the best features to be extracted, then it is done manually, usually driven by experience and previous results. According to \fig{img:classical_machine_learning}, this phase is referred to as {\it feature engineering}.

Data were acquired from \CHECK{XXX} subjects, during a period of \CHECK{YYY} months through Android smartphones worn in the right front pocket of the users' trousers. The following smartphones were used: Asus Zenfone 2, Samsung S3 Neo, Samsung S4, LG G2, LG G4 and a Google Nexus 5. Several acquisition sessions of about five minutes were performed for each subject, in variable conditions, e.g., with different shoes and clothes. We asked each subject to walk as he/she felt comfortable with, to mimic real world scenarios. For the data acquisition, we developed an Android inertial data logger application, which saves accelerometer, gyroscope and magnetometer signals into non-volatile memory and then automatically transfers them to an Internet server for further processing. The magnetometer signal is not used for identification purposes.

In \fig{fig:psd}, we plot the power of accelerometer and gyroscope signals at different frequencies through the Welch's method~\cite{Welch-67}, considering a full walking trace and setting the Hanning window length to $1$~s, with half window overlap. Most of the signal power is located at low frequencies, mostly below $40$~Hz (where the power is at least $30$~dB smaller than the maximum). The raw inertial signals were acquired using an average sample frequency ranging between $100$ and $200$~Hz (depending on the smartphone model), which is more than appropriate to capture most of the walking signal's energy. 

As the first block of our processing chain, due to the non-uniform sampling performed by the smartphone operating system, we apply a \CHECK{cubic} Spline interpolation to represent the input data evenly spaced points ($200$~points/second). Hence, a low pass Finite Impulse Response (FIR) filter with a cutoff frequency of $40$~Hz is used for denoising and to reduce the motion artefacts that may appear at higher frequencies. In fact, given the power profile of \fig{fig:psd}, the selected cutoff frequency only removes noise and preserves the relevant (discriminative) information about the user's motion.  

In the following, with $a_x(i)$ and $g_x(i)$ we respectively mean the filtered and interpolated acceleration and gyroscope time series along axis $x$, where $i=1,2,\dots$ is the sample number. The same notation holds for axes $y$ and $z$.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\columnwidth]{img/psd.eps}
	\caption{Power spectral density for accelerometer (continuous lines, one for each axis) and gyroscope (dashed lines) data.}
	\label{fig:psd}
\end{figure}

%The sampling frequency mean and standard deviation for the collected (raw) data are summarized in Tab.~\ref{tab:acquisition_performance}.
%\begin{table}[!ht]
%	\renewcommand{\arraystretch}{1.5}
%	\centering
%	\begin{tabular}{ c c c }
%		\hline
%		\textbf{Sensor type} & \textbf{Mean [Hz]} & \textbf{Sandard Deviation [Hz]} \\
%		\hline
%		Accelerometer & 119.16 & 0.01\\
%		Gyroscope & 204.35 & 39.22\\
%		Magnetometer & 60.06 & 5.47\\
%		\hline
%	\end{tabular}
%	\caption{Sampling frequency statistics for raw inertial data.}
%	\label{tab:acquisition_performance}
%\end{table}
%

\subsection{Extraction of Walking Cycles} 
\label{sec:cycle_extraction}

For the extraction of cycles we use a template-based and iterative method that solely considers the accelerometer's magnitude signal. This is in fact inherently invariant to the rotation of the smartphone and, as such, allows for the precise assessment of walking cycles regardless of how the user carries the device in his/her front pocket. For each sample $i=1,2,\dots$ we compute the acceleration magnitude as:
\be
a_{\rm mag}(i) = (a_x(i)^2 + a_y(i)^2 + a_z(i))^{1/2} \, .
\ee

To identify the template, we must determine a reference point for each walking cycle. Inspired by~\CHECK{add reference}, we proceed as follows. We first pass $a_{\rm mag}(i)$ through a low-pass filter with cutoff frequency of $3$~Hz. Thus, we detect the first minimum of this filtered signal, whose index is referred to as $\overline{i}$. This minimum is then refined by looking at the original signal $a_{\rm mag}(i)$ in a neighbourhood of it $\overline{i}$ and picking the minimum value of $a_{\rm mag}(i)$ in that neighborhood. This identifies a new index $i^\star$ for which $a_{\rm mag}(i^\star)$ is a local minimum. As an example, in \fig{img:correlation_distance}, we show this minimum through a red vertical (dotted) line. Hence, we take a fixed neighborhood of $i^\star$, picking half a second of values before and after it, so that $i^\star$ resides in the exact center of it, see the two vertical blue (dotted) lines in  \fig{img:correlation_distance}. Now, the acceleration samples falling between the two blue lines define the first template, which we call $\pmb{T}$, with $|\pmb{T}| = N_s$~samples, where $N_s$ corresponds to the number of samples collected in one second.\footnote{$N_s$ is automatically adapted by the algorithm as a function of the sampling rate that we use for the pre-filtering block. For the examples in this paper we set it to $200$~Hz.}  

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\columnwidth]{img/first_template.eps}
	\caption{Template extraction using the accelerometer magnitude $a_{\rm mag}(i)$. The first template is the signal between the blue dashed vertical lines. The red dashed line in the center corresponds to $i^*$.}
	\label{img:first_template}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\columnwidth]{img/correlation_distance.eps}
	\caption{Correlation distance $\gamma(i)$ between $a_{\rm mag}(i)$ and the template $\pmb{T}$. Local minima identify the beginning of subsequent walking cycles.}
	\label{img:correlation_distance}
\end{figure}

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{img/orientation_change.eps}
	\caption{Raw accelerometer data from two different walks, acquired from a smartphone worn in the right front pocket with different orientations. Accelerometer data in the smartphone reference system $\pmb{a}_{x}$, $\pmb{a}_{y}$, $\pmb{a}_{z}$ (left), and after the transformation $\pmb{a}_{\xi}$, $\pmb{a}_{\psi}$, $\pmb{a}_{\zeta}$ (right). Our PCA-based transformation makes walking data rotation invariant, i.e., subject-specific gait patterns emerge in the new coordinate system (see the red colored patterns in the right plots).}
	\label{img:orientation_change}
\end{figure*}

%
The extracted template is then iteratively refined and, at the same time, used to identify subsequent walking cycles. To this end, we first define the following correlation distance, defined for any two real vectors $\pmb{u}$ and $\pmb{v}$ of the same size:
%
\begin{IEEEeqnarray}{ll}
\mathrm{corr\_dist}(\pmb{u},\pmb{v}) = 1 - \dfrac{(\pmb{u}-\bar{\pmb{u}}) \cdot (\pmb{v}-\bar{\pmb{v}})}{\Vert(\pmb{u}-\bar{\pmb{u}})\Vert \  \Vert(\pmb{v}-\bar{\pmb{v}})\Vert} \, .
\label{eq:correlation_distance}
\end{IEEEeqnarray}

The template is then convolved with the acceleration magnitude through the following equations, leading to a further metric $\gamma(i)$, where $i=1,2,\dots$ is the sample index:  

\begin{IEEEeqnarray}{rl}
\mathrm{vrect}(a_{\rm mag}(i)) & = (a_{\rm mag}(i), \dots, a_{\rm mag}(i+N_s-1))^T \nonumber \\
\gamma(i) & = \mathrm{corr\_dist}(\pmb{T}, \mathrm{vrect}(a_{\rm mag}(i))
\label{eq:gamma}
\end{IEEEeqnarray}

As can be seen from \fig{img:correlation_distance}, the function $\gamma(i)$ exhibits some local minima, that can be promptly identified through a suitable threshold-based search ($th$ in the figure). The indices corresponding to these minima correspond to optimal alignments between the template $\pmb{T}$ and the acceleration $a_{\rm mag}(i)$. In particular, the second of these identifies the beginning of the second gait cycle. Specifically: 1) the samples between the second and the third minima correspond to the second gait cycle, and 2) at the same time, these samples define a second template $\pmb{T}^\prime$. At this point a new template is obtained averaging the old $\pmb{T}$ and the new one $\pmb{T}^\prime$, as:
\be
\pmb{T} = \alpha \pmb{T} + (1-\alpha) \pmb{T}^\prime \, ,
\ee
where we used $\alpha=0.9$. The new template $\pmb{T}$ is used for the subsequent 

This step allows to obtain an increasingly robust template on each new cycle.

At the end of this phase a list of $M$ different values of $\overline{T}$ is available $\pmb{\overline{T}} = [\overline{T}_0,\overline{T}_1,...,\overline{T}_{M-1}]$, each corresponding to the starting point of one of the $M$ total cycles.
This values are then used to extract the $m$-th cycle samples $\mathbf{cyc}_m[n]$, as in \eq{eq:single_cycle_samples}, not only from the acceleration magnitude $\pmb{a}_{mag}$, but also from all the available accelerometer and gyroscope signals.
%
\begin{IEEEeqnarray}{ll}
\mathbf{cyc}_m = \pmb{s} \left[\ \overline{T}_{m-1} : \overline{T}_{m} \right]  \qquad   m = 1,\cdots ,M
\label{eq:single_cycle_samples}
\end{IEEEeqnarray}
where $\pmb{s}$ is one of available signals $\pmb{a}_{mag}$, $\pmb{a}_{x}$, $\pmb{a}_{y}$, $\pmb{a}_{z}$, $\pmb{g}_{mag}$, $\pmb{g}_{x}$, $\pmb{g}_{y}$ or $\pmb{g}_{z}$.
%

Note that the number of samples could differ from cycle to cycle, as it depends on the duration of subsequent walking steps. Hence, a normalization step is required to represent all the segments through the same (constant) number of points $N$, as this will be convenient for the following feature extraction and classification algorithms. Before doing this, however, a reference system transformation is performed to obtain a rotation invariant reference system, as we describe in the next subsection.

%\begin{algorithm}[h]
%	\KwIn{Acceleration magnitude $\pmb{a}_{\mathrm{mag}}$}
%	\KwOut{Cycles indexes list}
%	\caption{multiobjective DE}
%	initialize population $P = \left \{ X_{1}, ... , X_{N} \right \} $\;
%	\For( \emph{Evolutionary loop}){$g := 1$ to $G_{max}$}
%	{
%		Do things \;
%		Trim the population to size $N$ using nondominated sorting and diversity estimation \;
%	}
%\end{algorithm}

\subsection{Orientation Independent Transformation}
\label{sec:reference_system_transformation}

To evaluate the new orientation invariant coordinate system three orthogonal versors $\hat{\pmb{\xi}}$, $\hat{\pmb{\zeta}}$, $\hat{\pmb{\psi}}$ are to be found, whose orientation must be independent of that of the smartphone and aligned with gravity and the direction of motion. Our aim is to express accelerometer and gyroscope signals in a coordinate system that remains fixed during each walking cycle, with versor $\hat{\pmb{\zeta}}$ pointing up (and parallel to the user's torso), versor $\hat{\pmb{\xi}}$ pointing forward (aligned with the direction of motion) and $\hat{\pmb{\psi}}$ tracking the lateral movement and being orthogonal to the other two. This entails inferring the orientation of the mobile device carried in the front pocket from the acceleration signal acquired during the walk. To this end, we adopt a technique similar to those of~\cite{pca-heading-2009, heading-2015}.

Gravity is the main low frequency component in the accelerometer data, and will be our starting point for the transform. Although it is a constant vector, gravity  continuously changes when represented in the $(x,y,z)$ reference system of the smartphone, due to the user's mobility and the subsequent change of orientation of the device. So, even the gravity vector $\vec{\pmb{g}}$ is not constant when expressed through the smartphone coordinates. As the first axis of the new reference system, we consider the mean direction of gravity within the current walking cycle. Let $n_k$ be the number of samples in the current cycle $k$, with $k=1,2,\dots$. With $\pmb{a}_x$, $\pmb{a}_y$ and $\pmb{a}_z$ we mean the acceleration samples measured by the smartphone in the current cycle along the three axes $x,y$ and $z$, with $|\pmb{a}_x|=|\pmb{a}_y|=|\pmb{a}_z|=n_k$. The gravity vector $\vec{\pmb{g}}_{k}$ within cycle $k$ is thus estimated as:
%
\begin{IEEEeqnarray}{ll}
\vec{\pmb{g}}_{k} = \dfrac{1}{n_K} \left( \sum_{j=1}^{n_k}{\pmb{a}_x[j]}\ , \sum_{j=1}^{n_k}{\pmb{a}_y[j]}\ , \sum_{j=1}^{n_k}{\pmb{a}_z[j]}  \right)^T
\label{eq:g_mean_vector}
\end{IEEEeqnarray}
%
The first versor of the new system $\hat{\zeta}$, and relative projected components $\pmb{a}_{\zeta}$ and $\pmb{g}_{\zeta}$, are defined in \eqs{eq:gravity_versor1}{eq:gravity_versor2}.
%
\begin{IEEEeqnarray}{CC}
\hat{\zeta} = \dfrac{\vec{G}_{m}}{\Vert\vec{G}_{m}\Vert} \label{eq:gravity_versor1} \\[0.1cm]
\pmb{a}_{\zeta} = \vec{\pmb{a}} \cdot \hat{\zeta} \hspace{1cm} \pmb{g}_{\zeta} = \vec{\pmb{g}} \cdot \hat{\zeta} \label{eq:gravity_versor2}
\end{IEEEeqnarray}
%
where $\Vert\cdot\Vert$ is the L2-norm operator. By removing this component from the original accelerometer signal, we obtain data that is flattened on a plane ($\vec{\pmb{a}}_{f}$).
%
\begin{IEEEeqnarray}{l}
\vec{\pmb{a}}_{f} = \vec{\pmb{a}} - \pmb{a}_{\zeta}\ \hat{\zeta} \label{eq:acc_flat}
\end{IEEEeqnarray}
%
Analyzing this data, we observed that during a gait cycle $\vec{\pmb{a}}_{f}$ isn't uniformly distributed on the plane, but has a preferential direction along which there is the greatest excursion in acceleration data. So we choose this direction as the second axis of the new reference system, identified by the versor  $\hat{\xi}$. To obtain information about the directionality of the data, we use Principal Component Analysis (PCA) theory. PCA projects the data along the direction of maximum variation (highest variance) and is consistent with the observation that the highest variation in the horizontal plane will be parallel to the walking direction, this was successfully applied in~\cite{pca-heading-2009}. 

%Using this heuristic, we infer the vertical component. Now
%we project the accelerometer signal in the plane perpendicular
%to the vertical gravity vector (=horizontal plane).
%We apply principle component analysis on the projected
%data points (see Figure 1) to get the direction where the
%acceleration variations is greatest. This is the axis that is
%parallel to the walking direction. A


 First a normalization is performed (\eq{eq:acc_flat_norm}).
%
\begin{IEEEeqnarray}{l}
\vec{\pmb{a}}_{{f}_{\mathrm{norm}}} = \dfrac{\vec{\pmb{a}}_{f} - \mathrm{mean}\left(\vec{\pmb{a}}_{f}\right)}{\mathrm{std}\left(\vec{\pmb{a}}_{f}\right)}
\label{eq:acc_flat_norm}
\end{IEEEeqnarray}
%
Autocovariance matrix $\pmb{\Sigma}$ is then evaluated as in \eq{eq:cov_mat}.
%
\begin{IEEEeqnarray}{l}
\pmb{\Sigma} = \mathbb{E}\left[ \left( \vec{\pmb{a}}_{{f}_{\mathrm{norm}}} \right) \cdot  \left( \vec{\pmb{a}}_{{f}_{\mathrm{norm}}} \right)^T \right]
\label{eq:cov_mat}
\end{IEEEeqnarray}
%
%Being  $\vec{\pmb{a}}_{{f}_{norm}}$ a $[3\times N]$ matrix (each row is related to one axis data), covariance matrix has dimension $[3\times 3]$.
The eigenvalues and corresponding eigenvectors of $\pmb{\Sigma}$ are then evaluated. The eigenvector $\vec{v}$ associated with the maximum eigenvalue has a direction that minimize the variance of data projected along it (referred to as first PCA component). A scaling is then necessary to obtain the correct direction on the original data (\eq{eq:denorm}).
%
\begin{IEEEeqnarray}{l}
\vec{v}_n = \vec{v}\ \circ \mathrm{std}\left(\vec{\pmb{a}}_{f}\right)
\label{eq:denorm}
\end{IEEEeqnarray}
%
where $\circ$ is the entrywise product operator.
In classical PCA, also the mean value is restored. In this case, instead, the direction of the resulting vector must intersect that of the previous estimated versor $\hat{\zeta}$. Without restoring the mean, we are sure about this condition, and the intersection point will be necessarily the origin, that remain unchanged after reference system transformation. Likewise previous step, the versor of the second axis, and projected component, can be evaluated as in \eqs{eq:xi_versor1}{eq:xi_versor2}.
%
\begin{IEEEeqnarray}{CC}
\hat{\xi} = \dfrac{\vec{v}_n}{\Vert\vec{v}_n\Vert} \label{eq:xi_versor1} \\[0.1cm]
\pmb{a}_{\xi} = \vec{\pmb{a}} \cdot \hat{\xi} \hspace{1cm} \pmb{g}_{\xi} = \vec{\pmb{g}} \cdot \hat{\xi} \label{eq:xi_versor2}
\end{IEEEeqnarray}
%
Being $\hat{\xi}$ placed on a plane that is orthogonal to $\hat{\zeta}$, the two versors are also othogonal. The third axis is then obtained simply with a cross product (\eqs{eq:psi_versor1}{eq:psi_versor2}).
%
\begin{IEEEeqnarray}{CC}
\hat{\psi} = \hat{\zeta} \times \hat{\xi}  \label{eq:psi_versor1} \\[0.1cm]
\pmb{a}_{\psi} = \vec{\pmb{a}} \cdot \hat{\psi} \hspace{1cm} \pmb{g}_{\psi} = \vec{\pmb{g}} \cdot \hat{\psi} \label{eq:psi_versor2}
\end{IEEEeqnarray}
%
The new transformed accelerometer and gyroscope data ${\vec{\pmb{a}}_T=(\pmb{a}_{\xi}, \pmb{a}_{\psi}, \pmb{a}_{\zeta})}$ and ${\vec{\pmb{g}}_T = (\pmb{g}_{\xi}, \pmb{g}_{\psi}, \pmb{g}_{\zeta})}$, in addition with the magnitudes $\pmb{a}_{\mathrm{mag}}$ and $\pmb{g}_{\mathrm{mag}}$, are the result of the preprocessing phase.

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.8\textwidth]{img/CNN_architecture_journal.eps}
	\caption{CNN-based authentication framework.}
	\label{fig:CNN_architecture}
\end{figure*}

An example of this reference transformation is shown in \fig{img:orientation_change}, where the data of two different walks of the same person are plotted. Data were acquired carrying the phone in the right pocket with two different orientations. In the original signals the repetitive pattern on each axis is very different between the two walks; transformed signals, instead, exhibit very similar patterns, that are highlighted in the figure.

\subsection{Normalization}
\label{sec:normalization}

As the Android operating system is non-realtime, the sampling rate is not constant during the acquisitions and in general differs for each inertial sensor. Moreover, 
each cycle has a different duration, which depends on walking speed and stride length. So, considering the accelerometer and gyroscope data collected during a full walking cycle (after the cycle extraction block, see \sect{sec:cycle_extraction}), we remain with variable-size 3D acceleration and gyroscope vectors along each axis ($x$, $y$ and $z$, i.e., the smartphone coordinate system). 

Since feature extraction and classification algorithms require $N$-sized vectors, where $N$ is the fixed number of samples per walking cycle, a further adjustment is necessary. Assuming a maximum cycle duration of $\tau=2$~seconds, which corresponds to a very slow walk, and a signal bandwidth of $B=40$~Hz, a number of samples $N > 2 B \tau = 160$~samples/cycle would be required to avoid aliasing. We coped with this through a Spline interpolation to represent all walking cycles through vectors of $N=200$ samples each. Amplitude normalization has also been implemented, to obtain vectors with zero mean and unit variance (as this leads to better training and classification results). 

Hence, considering a full walking cycle, accelerometer and gyroscope vectors are respectively indicated as:  $\vec{\pmb{a}} = (\pmb{a}_x, \pmb{a}_y, \pmb{a}_z)$ and $\vec{\pmb{g}} = (\pmb{g}_x, \pmb{g}_y, \pmb{g}_z)$. In addition, we evaluate their magnitude vectors, defined as\footnote{All the operations in the following equation are element-wise.}
%
\begin{IEEEeqnarray}{ll}
&\pmb{a}_{\mathrm{mag}} = \sqrt{\pmb{a}_x^2+\pmb{a}_y^2+\pmb{a}_z^2} \label{eq:magnitude1} \nonumber \\
&\pmb{g}_{\mathrm{mag}} = \sqrt{\pmb{g}_x^2+\pmb{g}_y^2+\pmb{g}_z^2} \label{eq:magnitude2} \, .
\end{IEEEeqnarray}

This returns a total of eight $N$-sized vectors for each walking cycle, which are then inputted into the feature extraction and classification algorithms.  






